Optimal trading without optimal control

A hypothetical risk-neutral agent who trades to maximize the expected profit of the next trade will approximately exhibit long-term optimal behavior as long as this agent uses the vector $p = \nabla V (t, x)$ as effective microstructure alphas, where V is the Bellman value function for a smooth relaxation of the problem. Effective microstructure alphas are the steepest-ascent direction of V , equal to the generalized momenta in a dual Hamiltonian formulation. This simple heuristics has wide-ranging practical implications; indeed, most utility-maximization problems that require implementation via discrete limit-order-book markets can be treated by our method.

==> Macros.tex <==
% sets 
\def\R{\mathbb{R}}

% operators 
\def\diag{\operatorname{diag}}

\def\argmin{\mathop{\operatorname{argmin}}}
\def\argmax{\mathop{\operatorname{argmax}}}

\def\cor{\operatorname{cor}}
\def\cov{\operatorname{cov}}
\def\var{\operatorname{var}}
\def\vol{\operatorname{vol}}
\def\mean{\operatorname{mean}}
\def\cov{\operatorname{cov}}
\def\vec{\operatorname{vec}}
\def\grad{\operatorname{grad}}

\def\cond{{ \,\mid\, }}

% delimiters and parens 
\def\norm#1{ \| #1 \| }
\def\lrp#1{\left( #1 \right)}
\def\lrb#1{\left[ #1 \right]}
\def\abs#1{\left| #1 \right|}

\def\lrpbig#1{\big( #1 \big)} 
\def\lrpBig#1{\Big( #1 \Big)} 
\def\lrbrace#1{\left\{ #1 \right\}} 
\def\lrbraceBig#1{\Big\{ #1 \Big\}} 
\def\lrbBig#1{\Big[ #1 \Big]} 

\def\bbE{\mathbb{E}} 
\def\bbV{\mathbb{V}} 


% calligraphic letters 
\def\cA{\mathcal{A}}
\def\cS{\mathcal{S}}

\def\qopt{q_{\text{opt}}}

% norms 
\def\norm#1{ {\left\| #1 \right\| } }
\def\abs#1{ {\left| #1 \right| } }

\def\twovector#1#2{\bigg( \begin{matrix} #1 \\ #2 \end{matrix}\bigg)}

\def\argmax{\mathop{\text{argmax}}}
\def\advp{\mathrm{advp}}
\def\adv{\mathrm{adv}} 
\def\val{\mathrm{value}}

\def\WaitState{\mathfrak{w}}
\def\PassiveState{\mathfrak{p}}
\def\AggressiveState{\mathfrak{a}}

\newenvironment{Figure}
{\par\medskip\noindent\minipage{\linewidth}}
{\endminipage\par\medskip}



